An Optimal Algorithm for Certifying Monotone Functions

Given query access to a monotone function $f\colon\{0,1\}^n\to\{0,1\}$ with certificate complexity $C(f)$ and an input $x^{\star}$, we design an algorithm that outputs a size-$C(f)$ subset of $x^{\star}$ certifying the value of $f(x^{\star})$. Our algorithm makes $O(C(f) \cdot \log n)$ queries to $f$, which matches the information-theoretic lower bound for this problem and resolves the concrete open question posed in the STOC '22 paper of Blanc, Koch, Lange, and Tan [BKLT22]. We extend this result to an algorithm that finds a size-$2C(f)$ certificate for a real-valued monotone function with $O(C(f) \cdot \log n)$ queries. We also complement our algorithms with a hardness result, in which we show that finding the shortest possible certificate in $x^{\star}$ may require $\Omega\left(\binom{n}{C(f)}\right)$ queries in the worst case.

==> overview-old.tex <==
\section{Technical Overview}

\subsection{Algorithm for Certifying a Binary Monotone Function}

\paragraph{Setup} We describe our algorithm for finding a $C(f)$-size certificate for a binary-valued monotone function $f$ on an input $x^*$. Without loss of generality, we let $f(x^*)=1$.\footnote{It may be worth reading the notation section of the preliminaries, though the rest of the formal definitions should not be necessary.}

Let $S_{x^*}$ be the set of indices on which $x^*$ is 1. Note that $S_{x^*}$ is a valid certificate, but not necessarily small enough. Our final certificate will be a subset of $S_{x^*}$; without loss of generality, we will let $S_{x^*}=[r]$ for some $r\geq 0$. A certificate $S$ is \emph{minimal} if $f(x_S)=1$, but by removing an element of $S$ to obtain $P\subset S$, we always have $f(x_P)=0$ ($S=\emptyset$ if $f(0^n)=1$).

The first observation is that \emph{any minimal certificate $S$ has length $\leq C(f)$}. This follows because on the input $x_S$, one must witness all of $S$ to see that the function value is $1$. Thus, our goal is to find any minimal certificate. If $f(x_{\emptyset})=1$, our minimal certificate is $\emptyset$.

\mnote{I do think the next section can probably be simplified significantly, esp since I didn't realize the phrasing "find the smallest index for which this holds" lmao}
\paragraph{Finding the Minimal Certificate} We now add elements into our minimal certificate. We want to find $a_1$ such that $f(x_{[a_1-1]})=0$ but $f(x_{[a_1]})=1$ (the set $[0]=\emptyset$ since we are 1-indexing). In other words, we want to find the value $a$ at which the function ``transitions'' from $0$ to $1$. There is exactly one such transition since $f$ is monotone (and therefore increasing with $a$. This can be found by binary searching. The value $a_1$ is now the first element of our certificate. If $f(x_{a_1})=1$, then $a_1$ is a minimal certificate, since $f(x_\emptyset)=0$.

Otherwise, we repeat the procedure to find $a_2<a_1$ such that $f(x_{[a_2-1]\cup a_1})=0$ but $f(x_{[a_2]\cup a_1})=1$. 
This must exist because when $a_2=0$, $f(x_{[a_2-1]\cup a_1})=0$, but when $a_2=a_1-1$, we have $f(x_{[a_2-1]\cup a_1})=1$, so there must be a transition point. 
Then $a_2$ becomes the second element of our certificate. Now if $f(x_{\{a_1,a_2\}})=1$, then $\inbraces{a_1,a_2}$ is a minimal certificate, since $f(x_{\{a_1\}})=0$ by assumption, and $f(x_{\{a_2\}})=0$, because of the stronger statement that $f(x_{[a_1-1]})=0$ (and the function is monotone). Otherwise, we add another element to our certificate similarly.

To add the general $(i+1)$th element to our certificate, find $a_{i+1}$ such that $f(x_{[a_{i+1}-1]\cup a_1\ldots a_i})=0$ but $f(x_{[a_{i+1}]\cup a_1\ldots a_i})=1$. If we then have $f_{\inbraces{a_1\ldots a_{i+1}}}=1$, we must have that $\inbraces{a_1\ldots a_{i+1}}$ is a minimal certificate. This is because for any $j\leq i+1$, we know that for $P=[j-1]\cup a_1\ldots a_{j-1}$, $x_{P}=0$ and $P$ is a superset of $\inbraces{a_1\ldots a_{j-1},a_{j+1}\ldots a_{i+1}}$, so the value on that set must also be $0$.

This procedure eventually terminates with a certificate; we can repeat unless $a_i=1$, and if that's the case we must have a certificate already. Note that adding each element takes up to $O(\log{n})$ queries. Since the certificate is minimal, the procedure took less than $C(f)$ steps, so the final query complexity is $O(C(f)\log{n})$.
